Hiding the Rumor Source

Anonymous social media platforms like Secret, Yik Yak, and Whisper have emerged as important tools for sharing ideas without the fear of judgment. Such anonymous platforms are also important in nations under authoritarian rule, where freedom of expression and the personal safety of message authors may depend on anonymity. Whether for fear of judgment or retribution, it is sometimes crucial to hide the identities of users who post sensitive messages. In this paper, we consider a global adversary who wishes to identify the author of a message; it observes either a snapshot of the spread of a message at a certain time, sampled timestamp metadata, or both. Recent advances in rumor source detection show that existing messaging protocols are vulnerable against such an adversary. We introduce a novel messaging protocol, which we call adaptive diffusion, and show that under the snapshot adversarial model, adaptive diffusion spreads content fast and achieves perfect obfuscation of the source when the underlying contact network is an infinite regular tree. That is, all users with the message are nearly equally likely to have been the origin of the message. When the contact network is an irregular tree, we characterize the probability of maximum likelihood detection by proving a concentration result over Galton-Watson trees. Experiments on a sampled Facebook network demonstrate that adaptive diffusion effectively hides the location of the source even when the graph is finite, irregular and has cycles.

==> general_spies.tex <==
	\begin{table*}
\begin{center}
    \begin{tabular}{ | l | l | l | l |}
    \hline
    Spy Probability $p$ & Adaptive Diffusion  & Diffusion ($q=0.1$) & Diffusion ($q=0.5$) \\ \hline 
\hline
    0.05 &  \textbf{0.10 $\pm$ 0.03} & 0.83 $\pm$ 0.05 & 0.99 $\pm$ 0.01 \\ \hline
    0.10 &  \textbf{0.14 $\pm$ 0.05} & 0.86 $\pm$ 0.05 & 1.00 $\pm$ 0.00 \\ \hline
    0.15 &  \textbf{0.17 $\pm$ 0.05} & 0.90 $\pm$ 0.04 & 1.00 $\pm$ 0.00 \\ \hline
    \end{tabular}
\caption{Probability of detection  over the Facebook dataset \cite{viswanath-2009-activity}, with 95$\%$ confidence intervals.}
\label{tab:fb}
\end{center}
\end{table*}


\subsection{Irregular Trees}
\label{sec:irregular}


Here, we consider tree networks with nonuniform node degrees.
Regardless of spreading protocol or underlying network structure, the message always propagates over a tree superimposed on the underlying contact network. 
The probability of detection over 
\emph{irregular} trees is therefore closely tied to performance over general graphs.
ML estimation over irregular trees is more straightforward than in Section \ref{sec:irregular_trees}, primarily because we use the specialized Tree Protocol, which always places the source at a leaf node.

\begin{propo}\label{prop:irr}
Suppose the underlying contact network $G(V,E)$ is an irregular tree with the degree of each node larger than one. One node $v^*\in V$ starts spreading a message at time $T=0$ according to Protocol \ref{alg:tree}. Each node $v\in V$, $v\neq v^*$ is a spy with probability $p$. Let $U$ denote the set of feasible candidate sources obtained by estimation Algorithm \ref{alg:ml_est}. Then the maximum likelihood estimate of $v^*$ given $U$ is 
\begin{equation}
\hat v_{\rm ML}=\argmax_{u\in U} \frac{1}{\deg(u)} \prod_{v\in \mathcal P(u,\ell_{min})\backslash \{u,\ell_{min}\}}\frac{1}{\deg(v)-1}\;,
\label{eq:irr}
\end{equation}
where $\ell_{min}$ is the lowest-level pivot node, $\mathcal P(u,\ell_{min})$ is the unique shortest path between $u$ and $\ell_{min}$, and $\deg(u)$ denotes the degree of node $u$.
(Proof in Section \ref{sec:proofs})
\end{propo}
%The proof can be found in Section \ref{sec:irr} of the Supplemental Materials. %The only randomness in adaptive diffusion comes from choosing spine nodes, so the proof shows that for each candidate source, we need only compute the probability of observing a given spine up to the minimum-level pivot node $\ell_{min}$. The expression in \ref{eq:irr} is precisely this probability.


\subsection{Real-World Networks}\label{sec:facebook_spies}
Equipped with a maximum-likelihood estimator for irregular trees, 
we can evaluate adaptive diffusion over a real dataset---namely, the Facebook social graph from \cite{viswanath-2009-activity} used in Section \ref{sec:irregular_trees}---against a spy-based adversary. 
 %Over this underlying connectivity network, we ran 
 We simulate adaptive diffusion and regular diffusion for $q\in\{0.1,0.5\}$. We evaluate a lower bound on the probability of detection under diffusion using the first-spy estimator; for adaptive diffusion, we use a slightly-modified version of the ML estimator in Proposition \ref{prop:irr}, that accounts for cycles in the underlying graph.
Table \ref{tab:fb} lists the probability of detection averaged over 200 trials, for $p$ up to 0.15.\footnote{We chose this value because at its height, the Stasi employed 11 percent of the population as spies \cite{koehler1999stasi}.} 
Not only does adaptive diffusion hide the source better than diffusion, its probability of detection in practice is close to the fundamental lower bound of $p$.
This is likely because the mean node degree in the dataset is 25, so high-degree asymptotics are significant.
It is common for social networks to have degree distributions that skew large \cite{clauset2009power}.
Additionally, while adaptive diffusion can never reach all nodes in a tree, cycles in the Facebook graph allow it to reach 81$\%$ of nodes within 20 timesteps. %The spreading rate of diffusion depends on $q$. 






